Deep Model Fusion: A Survey

Deep model fusion/merging is an emerging technique that merges the parameters or predictions of multiple deep learning models into a single one. It combines the abilities of different models to make up for the biases and errors of a single model to achieve better performance. However, deep model fusion on large-scale deep learning models (e.g., LLMs and foundation models) faces several challenges, including high computational cost, high-dimensional parameter space, interference between different heterogeneous models, etc. Although model fusion has attracted widespread attention due to its potential to solve complex real-world tasks, there is still a lack of complete and detailed survey research on this technique. Accordingly, in order to understand the model fusion method better and promote its development, we present a comprehensive survey to summarize the recent progress. Specifically, we categorize existing deep model fusion methods as four-fold: (1) "Mode connectivity", which connects the solutions in weight space via a path of non-increasing loss, in order to obtain better initialization for model fusion; (2) "Alignment" matches units between neural networks to create better conditions for fusion; (3) "Weight average", a classical model fusion method, averages the weights of multiple models to obtain more accurate results closer to the optimal solution; (4) "Ensemble learning" combines the outputs of diverse models, which is a foundational technique for improving the accuracy and robustness of the final model. In addition, we analyze the challenges faced by deep model fusion and propose possible research directions for model fusion in the future. Our review is helpful in deeply understanding the correlation between different model fusion methods and practical application methods, which can enlighten the research in the field of deep model fusion.

==> tex/other.tex <==


\begin{table}
\centering
\caption{Notations.}
\label{table1}
\vspace{0.5em}
\begin{tabular}{c c c} 
\toprule
 Components & Definition   \\ 
 
   
   \midrule
 

$W_{i}$ & neural network& \\
$\theta_{i}$ & neural network`s parameters \\
$\mathcal{L}$ &loss function\\
$x$ & the input of the neural network\\


 \bottomrule
\end{tabular}
\end{table}



==> tex/preliminary.tex <==
\section{Preliminary} 


%ensemble -survey-2018
This theorem has two major limitations: The assumption that the votes are independent and that there are only two possible outcomes. In his 2004 book, The Wisdom of Crowds: Why the Many Are Smarter than the Few and How Collective Wisdom Shapes Business, Economies, Societies and Nations, James Michael Surowiecki elaborates upon this notion. He describes how combining information from different sources results in decisions that are often better than those of a single individual


\begin{table}
\begin{tabular}{l c c c c c} 
 \hline
- &  Method & Ref. & Intro   \\ 
 \hline
\multirow{4}*{-}
& WHN & \cite{wang2013co}  &  -
\\

%output of a single source model is utilized as the features to guide the target model training
& FMR & -  &  use output of a single model as the features to guide the target model 
\\

&  $PM^{2}R$ & \cite{xiang2017modal} & utilizing consistency on different modalities  \\

&  MMR & \cite{lou2019towards} & reuse multiple source models  \\


& NMMR & \cite{luo2022nonlinear} & take advantage of the nonlinear relationship  \\
  


\multirow{3}*{-} 

& HMR & \cite{wu2019heterogeneous}  &  output of local models are utilized to derive a global model, the data can be non-i.i.d

\\


		~ &   HMR for ML & \cite{tang2023improving}   & -\\

 &   RKME & \cite{wu2021model}   &  improves the zero-shot test accuracy, but complicated model is required\\
       
  &   RKHS & \cite{wu2021model}   &  -\\    




 \hline
\end{tabular}
\caption{Multi-model Reuse Method
}
\label{Table1}
\end{table}




%
\begin{table}\centering
\begin{tabular}{l c c c c} 
 \hline
  &  Method & Ref. & Out of domain & In domain   \\ 
 \hline
\multirow{9}*{}

& SGD &   &   &  \\
& SWA & \cite{izmailov2018averaging} &  $85.9\pm0.1$ & $97.1\pm0.1$ \\
& EMA & \cite{polyak1992acceleration,szegedy2016rethinking} &  $85.5\pm 0.4$ & $97.0\pm 0.1$   \\

& ERM(Empirical Risk Minimization & & & \\



% improve the (OOD) generalization performance of DNN

& SWAD & \cite{cha2021swad}  & $87.1\pm0.2$ &$97.7\pm0.1$\\

 \hline
\end{tabular}
\caption{Comparison between generalization methods on PACS\cite{li2017deeper}. The scores are averaged over all settings using different target domains
}
\label{Table1}
\end{table}


%FL table
%1
\begin{table}[!h] \small 
\centering

\begin{tabular}{c|c|ccc}
  \hline
    \multicolumn{2}{c|}{-} & - & Ref. & - \\

%multi-teacher
  \hline
    \multirow{5}{*}{-}
      & \multirow{3}{*}{1} & FedDF & \cite{Lintao2020FedDF} & -\\
	  \cline{3-5}
		&  & FedMR &- &-	\\
    \cline{3-5}
		&  & - & - &-	\\

%type 2
  \cline{2-5}
      & \multirow{2}{*}{2} & - & - & -\\
	  \cline{3-5}
		&  & - & - &-	\\

%multiple-stu    
\cline{2-5}
     \hline
    \multirow{4}{*}{2} 
 & \multirow{2}{*}{3} & - &-& -\\
 \cline{3-5}
		&  & - & - &-	\\
	 
%type2
\cline{2-5}
 & 4 & - & -& -\\

%  \cline{2-5}
 %\hline
  %  \multicolumn{2}{c|}{Other Alignment 1} 
   % & - & - & -  \\    
%  \hline
 %   \multicolumn{2}{c|}{Other Alignment 2} & \multicolumn{3}{c}{-}\\
\hline
 \end{tabular}
 \caption{FL} \label{mult}
 \end{table}
%1


%
\begin{table}[!h] \small 
\centering

\begin{tabular}{c|c|ccc}
  \hline
    \multicolumn{2}{c|}{Distillation mode} & - & Ref. & - \\

%multi-teacher
  \hline
    \multirow{5}{*}{\makecell[c]{Merge multiple\\ teachers}}
      & \multirow{4}{*}{1} & FedDF & \cite{Lintao2020FedDF} &  \makecell[c]{addresses the quality loss issue\cite{hsieh2020non} of $BN$, break the \\ knowledge barriers among heterogeneous client models}\\
	
  %edit
  \cline{3-5}
		&  & EN$D^{2}$ & \cite{malinin2019ensemble} & Bayesian	\\
    \cline{3-5}
		&  & AE-KD & \cite{du2020agree} & \makecell[c]{regard the ensemble knowledge distillation\\ as a multi-objective optimization problem}	\\
\cline{3-5}
		&  & FedFTG &   \cite{zhang2022fine} & -	\\

	
%type 2
%  \cline{2-5}
   %   & \multirow{2}{*}{2} & - & - & -\\
	  %\cline{3-5}
		%&  & - & - &-	\\

%multiple-stu    
\cline{2-5}
     \hline
    \multirow{4}{*}{\makecell[c]{Merge multiple\\ students}} 
 & \multirow{4}{*}{3} & Batch Ensemble & \cite{wen2020batchensemble}& \makecell[c]{mini-batch friendly, parallelizable within\\a device, minor memory overhead }\\
 %$\bar{W}_{i}=W \circ F_{i} \text {,  } F_{i}=r_{i} s_{i}^{\top}$ \\

	 \cline{3-5} 
  &  & - & \cite{mariet2020distilling} &-	\\
	  \cline{3-5} 
  &  & Hydra  & \cite{tran2020hydra} &\makecell[c]{ improves distillation performance while capturing\\ the uncertainty behavior of the original ensemble }	\\ 
  
  \cline{3-5} 
  &  & LatentBE  & \cite{nam2022improving} &-	\\ 



%type2
%\cline{2-5}
 %& 4 & - & -& -\\

%  \cline{2-5}
 %\hline
  %  \multicolumn{2}{c|}{Other Alignment 1} 
   % & - & - & -  \\    
%  \hline
 %   \multicolumn{2}{c|}{Other Alignment 2} & \multicolumn{3}{c}{-}\\
\hline
 \end{tabular}
 \caption{Classification of KD according to the differences of the aggregated objects} \label{mult}
 \end{table}
%

